Towards Better Analysis of Deep Convolutional Neural Networks

Deep convolutional neural networks (CNNs) have achieved breakthrough performance in many pattern recognition tasks such as image classification. However, the development of high-quality deep models typically relies on a substantial amount of trial-and-error, as there is still no clear understanding of when and why a deep model works. In this paper, we present a visual analytics approach for better understanding, diagnosing, and refining deep CNNs. We formulate a deep CNN as a directed acyclic graph. Based on this formulation, a hybrid visualization is developed to disclose the multiple facets of each neuron and the interactions between them. In particular, we introduce a hierarchical rectangle packing algorithm and a matrix reordering algorithm to show the derived features of a neuron cluster. We also propose a biclustering-based edge bundling method to reduce visual clutter caused by a large number of connections between neurons. We evaluated our method on a set of CNNs and the results are generally favorable.

==> data.tex <==
% !TEX root = EvoTree-KDD.tex

\section{Background: }\label{sec:data}



==> discussion.tex <==
\section{Discussion}

After the case studies, we held an discussion with the expert team to collect their feedbacks.
Overall, CNNVis is well received by them.

All the experts appreciated CNNVis as a research tool to help them understand, diagnose, and refine CNNs.
They strongly requested us to open the source code and expressed their will to use CNNVis in their future research. 
Expert $E_2$ commented that, "It is often criticized that building a high-quality CNN is like a `black magic' because we do not know when and whether it will be beneficial to add a specific technique to the current model.
Now I have a toolkit that enables directly analysis [of a CNN].
It can help me quickly find the problem and trigger me to apply corresponding technique [to solve the problem]."

%The experts were impressed by the interactions provided by CNNVis.
%Expert $E_4$ especially favored the interactive clustering result modification. 
%She said that, ``Currently, if I want to debug a model, I have to ''

The experts also suggested several improvements.
The target user of CNNVis is experts with domain knowledge.
The experts believed that CNNVis can also be used to illustrate the working mechanism of a CNN for average users or researchers from other fields.
They suggested a more intuitive visual design as well as removing the debug information.
%Expert $E_6$ said, ``Besides refining or debugging a model, this toolkit can help ''

In addition, the experts expressed the need to integrate CNNVis with the training process.
Currently, we take a snapshot of the model in the training process as the input of CNNVis.
Expert $E_5$ commented that, ``Now, if I want to examine a snapshot of the model, I have to load the snapshot to the toolkit.
It is better to automatically update the visualization during the training process.''

Moreover, the experts recommended us to extend CNNVis to other kinds of deep models that can not be formulated as a DAG, such as recurrent neural network (RNN).
They also suggested that CNNVis should provide flexible interfaces so that they can customize CNNVis to their needs.
For example, expert $E6$ wants to implement his own clustering methods for neurons. 

\mengchen{Mengchen: other problems of CNNVis: can not handle large number of classes, image patches are sometimes too small to view}

%whose research interest is human face classification, said, ``For a model ''
%7. on other network structure, eg RNN
%3. other tasks such as detection

%large number of classes.

%Another possible improvement is that CNNVis experts want to implement their own algorithm.




% identity-related attributes
%(IA), such as gender, race, and shapes of facial components,
%as well as the identity non-related attributes
% such as expression, lighting, and photo quality.

%Another possible improvement is that

%1. image patches are sometimes too small to view.
%510. lense for large image

%In addition, all the experts requested us to open the source code and make the tool public.
%In addition, expert $E_6$ and $E_4$ requires to able to view the

%other information
%6. activation distribution, instead of average

%The automatically propose advise


%2. surprised that it can improve the performance for such a gap. -> case 3
%3. Hinge loss is hard to train, is commonly known, but they do not know how to solve that. -> case 2
%6. fast handle new data -> case 1

%7. interesting interaction


%Improvement

%2. implement their own clustering methods

%4.
%5. merged with Caffe



%9. small network can trial and error







==> evaluation.tex <==
%\section{Evaluation}
\section{Quantitative Evaluation}\label{sec:evaluation}

%We \kgsedit{conduct a quantitative evaluation of} the effectiveness of our MRG computation and incremental ranking update algorithm.
%In this section, we quantitatively evaluated the effectiveness of our MRG computation and incremental ranking update algorithm.
In this section, we quantitatively \doc{evaluate} the effectiveness of our MRG computation and incremental ranking update algorithm.

\subsection{MRG Computation}\label{sec:computation}

To evaluate the performance of our MRG computation based on the Monte Carlo sampling method, we compared it with the matrix-based method proposed in~\cite{Duan2012_coling}.
%We \kgsedit{used} two Twitter datasets \kgsedit{, namely, Shutdown and Ebola,} in the experiments.
We used two Twitter datasets in the experiments: government shutdown and Ebola outbreak.
The shutdown dataset contains tweets on the 2013 US government shutdown (5,132,510 tweets from Oct. 1 to Oct. 16, 2013), which were collected by using queries such as ``shutdown.''
The Ebola dataset contains tweets on the Ebola outbreak (1,425,017 tweets from Jan. 1 to Dec. 25, 2014), which were collected by using queries such as ``ebola.''
%We implemented both our algorithm and the baseline algorithm in C\#.
%All experiments \kgsedit{are} conducted on a PC with a 3.1GHz CPU and 16 GB RAM.
All experiments were conducted on a PC with a 3.1GHz CPU and 16 GB RAM.\looseness=-1

\begin{table}[b]
\vspace{-3mm}
  \centering
  \centering \scalebox{0.85}{
    \begin{tabular}{|c|c|c|c|c|c|c|c|}
    \hline
    \multirow{2}[4]{*}{Dataset} & \multirow{2}[4]{*}{n-Prec} & \multicolumn{2}{c|}{Post} & \multicolumn{2}{c|}{User} & \multicolumn{2}{c|}{Hashtag} \\
\cline{3-8}          &       & Base  & Ours  & Base  & Ours  & Base  & Ours \\
    \hline
    \multirow{4}[8]{*}{Shutdown} & 10-Prec & 1.000     & 1.000     & 0.900   & 1.000     & 1.000     & 1.000 \\
\cline{2-8}          & 50-Prec & 0.920  & 0.940  & 0.940  & 0.960  & 0.960  & 0.960 \\
\cline{2-8}          & 100-Prec & 0.870  & 0.930  & 0.850  & 0.920  & 0.910  & 0.930 \\
\cline{2-8}          & 200-Prec & 0.840  & 0.900   & 0.845 & 0.875 & 0.855 & 0.860 \\
    \hline
    \multirow{4}[8]{*}{Ebola} & 10-Prec & 1.000     & 1.000     & 0.800   & 1.000     & 1.000     & 1.000 \\
\cline{2-8}          & 50-Prec & 0.840  & 0.860  & 0.660  & 0.780  & 0.880  & 0.920 \\
\cline{2-8}          & 100-Prec & 0.770  & 0.840  & 0.660  & 0.730  & 0.870  & 0.880 \\
\cline{2-8}          & 200-Prec & 0.765 & 0.800   & 0.610  & 0.710  & 0.860  & 0.870 \\
    \hline
    \end{tabular}%
    }
    \caption{%Compare the MRG computation method with the  baseline using top-n precision for posts, users, and hashtags.
\doc{Comparison of} the MRG computation method with the  baseline using top-n precision for posts, users, and hashtags.}
     %on both the shutdown and Ebola datasets. Our method can retrieve more relevant items than the baseline method.}
  \label{tab:Retrieval_Result_Evaluation}%
  \vspace{-2mm}
\end{table}%

%\kgsedit{The huge amount of posts meant we could not} label all of them.
%There were too many posts, users or hashtags and we could not label all of them.
There were too many posts, users\doc{,} or hashtags and we could not label all of them.
\kgsedit{Thus,} we did not report the recall in our evaluation.
%Thus we did not report the recall in our evaluation.
In this evaluation, we used top n-precision (n-Prec) as the evaluation measure.
%Top n-precision is the percentage of the relevant items among the top-n ranked items.
Top n-precision is the percentage of the \shimei{correctly retrieved} items among the top-n ranked items.
%This measure is often used when the recall is hard to be calculated~\cite{Chandramouli2007co}.
This measure is often used when the recall is hard to \shimei{calculate}~\cite{Chandramouli2007co}.
%\kgsedit{We calculate} the top 10, 50, 100,\kgsedit{and} 200-precision for posts, users, and hashtags \kgsedit{to fully compare the two algorithms}.
%To fully compare the two algorithms, we calculated the top 10, 50, 100, 200-precision for posts, users, and hashtags, respectively.
To fully compare the two algorithms, we calculated the top 10, 50, 100, \doc{and} 200-precision for posts, users, and hashtags, respectively.
%We invited two PhD students to evaluate the retrieval results, who majored in data mining and are familiar with the datasets.
\revision{We invited two PhD students who majored in data mining and are familiar with the datasets to evaluate the retrieval results.}
%They labeled the \kgsedit{results individually} and resolved their differences by discussion.
They labeled the \kgsedit{results individually} and resolved \doc{the} differences \doc{via} discussion.
%They individually labeled the result and resolved their differences by discussion.
The results are shown in Table~\ref{tab:Retrieval_Result_Evaluation}.
Overall, our algorithm performed better than the baseline on both datasets.
%We inspect the top 10 retrieved items by both methods.
We \doc{inspected} the top 10 retrieved items \doc{with} both methods.
%In general, \kgsedit{the retrieved items} are quite accurate. \kgsedit{However,} the baseline \kgsedit{had} one mistake in the top 10 users selected from the shutdown dataset. It overestimated the importance of a user called @governmentclosd who posted \kgsedit{a significant number of} tweets with \kgsedit{a number of} hashtags.
In general, \kgsedit{the retrieved items} \doc{were} quite accurate. \kgsedit{However,} the baseline \kgsedit{had} one mistake in the top 10 users selected from the shutdown dataset. It overestimated the importance of a user called @governmentclosd\doc{,} who posted \kgsedit{a significant number of} tweets with \kgsedit{a number of} hashtags.
%In general, they are quite accurate. But the baseline made one mistake in the top 10 users selected from the Shutdown dataset.It overestimated the importance of a user called @governmentclosd who posted a lot of tweets with a lot of hashtags.
\kgsedit{However,} this user did not have many followers and his/her tweets were seldom retweeted.
%But this user did not have many followers and his/her tweets were seldom retweeted.
In contrast, our algorithm can avoid this mistake by taking a user's authority into consideration.
%In contrast, our algorithm can avoid this mistake by taking a user's \shimei{popularity} into consideration.
\kgsedit{The baseline algorithm also had similar mistakes in the} Ebola dataset.
%Similarly, in the Ebola dataset, the baseline algorithm made similar mistakes.

% Table generated by Excel2LaTeX from sheet 'Shimei'



\subsection{Incremental Ranking Update}
%\revision{Since the incremental ranking update algorithm only calculate the statistics of the changed random walks, it is more efficient than the full update.}
\revision{Since the incremental ranking update algorithm only calculate\shimei{s} the statistics of the changed random walks, it is more efficient than the full update.}
In this section, we conducted an experiment to \kgsedit{highlight} the effectiveness of our incremental ranking update algorithm.
%We also conducted an experiment to show the effectiveness of our incremental ranking update algorithm.

%\revision{First, we demonstrate the incremental algorithm converges quickly. To this end, we} invited two analysts to use our system. One analyst \kgsedit{worked} on the Shutdown dataset \kgsedit{while} the other \kgsedit{worked} on the Ebola dataset.
\revision{First, we demonstrate \shimei{that} the incremental algorithm converges quickly. To this end, we} invited two analysts to use our system. One analyst \kgsedit{worked} on the Shutdown dataset \kgsedit{while} the other \kgsedit{worked} on the Ebola dataset.
%We invited two analysts to use our system. One analyst works on the Shutdown dataset and the other works on the Ebola dataset.
\kgsedit{They updated the ranking incrementally based} on the initial retrieval \kgsedit{results.}
%Based on the initial retrieval result they incrementally updated the ranking.
%In the updating process, when the analyst found the ranking score of an item \kgsedit{to be underestimated,} he \revision{increased} its ranking score according to his knowledge and vice versa.
%In the updating process, when the analyst found the ranking score of an item \kgsedit{to be underestimated,} he \revision{increased} its ranking \shimei{score and} vice versa.
\doc{During} the \doc{update} process, when the analyst found \doc{a} ranking score of an item \doc{was} \kgsedit{underestimated,} he \revision{increased} its ranking \shimei{score and} vice versa.
%In the updating process, when the analyst found the ranking score of an item is underestimated he increases its ranking score according to his knowledge and vice versa.
%When he finds an overestimated item he decreases the ranking score of it.
After each \kgsedit{update,} we re-calculated the top-200 precision for posts, users, and hashtags.
%After each update we re-calculated the top-200 precision for posts, users, and hashtags.
After \kgsedit{five updates,} we observed that results were nearly unchanged from the last update. \kgsedit{Hence, we allowed them to} stop the process.
%After 5 updates we observed that results were nearly unchanged from the last update. So we let them stop the process.
The results after each update are listed in Table~\ref{tab:Incremental_Ranking_Update_Evaluation}.

Table~\ref{tab:Incremental_Ranking_Update_Evaluation} \kgsedit{shows that} the retrieval results \kgsedit{improved gradually} as they interactively modified the ranking scores.
%From Table~\ref{tab:Incremental_Ranking_Update_Evaluation}, we can see that the retrieval results gradually improve as they interactively modify the ranking scores.
%This result verifies that our method can refine the retrieval results \kgsedit{interactively} by integrating analysts' feedback.
%This result verifies that our method can interactively refine the retrieval results by integrating analysts' feedback.
This result verifies that our method can interactively refine the retrieval results by integrating \doc{analyst} feedback.

%We can further observe that after some updates, the performance of more than one types of items change too.
%We can further observe that after some updates, the performance of more than one types of items change\shimei{d} too.
We can further observe that after some updates, the performance of more than one \doc{type} of \doc{item} change\shimei{d} \doc{as well}.
For example, after changing the first item in the Ebola dataset, the performance of the retrieved posts, users, and hashtags all increased. This result confirmed the effectiveness of the MRG model and the developed computation method.

%We used the retrieval result of our method as the starting point. At each step we modified the ranking score of an item according to our prior knowledge. In both datasets, we increase the ranking scores for two items and decrease those for three. Thus the total number of updates  is 5 on each dataset. We documented the changes of 200-precision for posts, users and hashtags. The changes are shown in Table.

%\shimei{Mengchen: would you please explain a little bit more about prior knowledge. it is unclear how you increase and decrase the scores. over all, evaluation 2 is not very clear. Would you please first summarize what you want to evaluate, what your expectations/hypotheses are and whether the results support or refute your hypotheses.}

% Table generated by Excel2LaTeX from sheet 'Shimei'
\begin{table}[htbp]
  \centering
    \begin{tabular}{|c|c|c|c|c|c|c|}
    \hline
    \multirow{2}[4]{*}{Update} & \multicolumn{3}{c|}{Ebola} & \multicolumn{3}{c|}{Shutdown} \\
\cline{2-7}          & Post & User & Hashtag & Post & User & Hashtag \\
    \hline
    0     & 0.800   & 0.710  & 0.870  & 0.900   & 0.875 & 0.860 \\
    \hline
    1     & 0.815 & 0.715 & 0.875 & 0.910  & 0.875 & 0.865 \\
    \hline
    2     & 0.840  & 0.720  & 0.880  & 0.915 & 0.875 & 0.865 \\
    \hline
    3     & 0.855 & 0.720  & 0.885 & 0.925 & 0.885 & 0.875 \\
    \hline
    4     & 0.855 & 0.720  & 0.890  & 0.925 & 0.885 & 0.880 \\
    \hline
    5     & 0.855 & 0.720  & 0.895 & 0.925 & 0.885 & 0.885 \\
    \hline
    \end{tabular}%
    \caption{Evaluation of our incremental ranking update algorithm.
    %\kgsedit{We performed a total of five} updates for both the shutdown \kgsedit{and} Ebola \kgsedit{datasets}.
    The changes are evaluated by top-200 precision.
    %The row with 0 update contains the initial \kgsedit{results}.
    The row with 0 \doc{updates} contains the initial \kgsedit{results}.}
%    \caption{Evaluation of our incremental ranking update algorithm. Totally we made 5 updates for both the Shutdown and the Ebola dataset. The changes are evaluated by top-200 precision for posts, users and hashtags. The row with 0 update contains the initial result.}
  \label{tab:Incremental_Ranking_Update_Evaluation}%
  \vspace{-2mm}
\end{table}%

%\revision{Second, we illustrate that the ranking result of the incremental update algorithm is the same with that of the full update.
%The statistics of the random walks that contain changed elements of the affinity matrix need to be updated when the ranking of one item is modified.
%remove by Shimei
%Since the incremental update algorithm can fully updated the statistics of the changed random walks, the incremental update achieves the same result as the full update.}
%\revision{\shimei{Second, since} the incremental update algorithm can fully updated the statistics of the changed random walks, the incremental update achieves the same \shimei{ranking} result as the full update \shimei{algorithm}.}
\revision{\shimei{Second, since} the incremental update algorithm can fully \doc{update} the statistics of the changed random walks, the incremental update achieves the same \shimei{ranking} result as the full update \shimei{algorithm}.}
%In this section we provide quantitative evaluations of MRG computation and incremental ranking update algorithm.
%
%%In this section we provide quantitative evaluations of MRG computation and incremental ranking update algorithm.
%%
%\subsection{Uncertainty Measure}
%To evaluate the performance of our retrieval model, we compared it with the Duan’s baseline algorithm proposed by ~\cite{Duan2012_coling}. We implement our algorithm and the baseline algorithm by C\#. All experiments are done on a PC with CPU@3.1GHz and 16 GB RAM.
%We use two datasets for the experiments. Shutdown and Ebola. Shutdown dataset contains 658385 tweets containing word shutdown during the government shutdown period from October 1, 2013 to October 16, 2013. Ebola dataset contains 1425017 tweets containing word ebola from January 1, 2014 to December 25, 2014.
%As there are too many posts we cannot label all the important posts, users or hashtags. Thus we cannot compare the recall. In this scenario we use n-precision for evaluation. N-precision is the precision of the top n ranked items. For a positive number N it is defined as ratio of the number of correct retrieved items among top N items and N. To fully compare the two algorithms we calculate 10, 50, 100, 200-precision of posts, users and hashtags. We invite two PhD students to do the annotation. They firstly individually labeled the dataset and then resolved the difference by discussion. The results are shown in Table .
%
%% Table generated by Excel2LaTeX from sheet 'Tables'
%\begin{table}[htbp]
%  \centering
%  \caption{Add caption}
%    \begin{tabular}{|c|c|c|c|c|c|c|c|}
%    \hline
%    \multicolumn{2}{|c|}{\multirow{2}[4]{*}{}} & \multicolumn{2}{c|}{Post} & \multicolumn{2}{c|}{User} & \multicolumn{2}{c|}{Hashtag} \\
%\cline{3-8}    \multicolumn{2}{|c|}{} & Duan's & Ours  & Duan's & Ours  & Duan's & Ours \\
%    \hline
%    \multirow{4}[8]{*}{shutdown} & 10-Precision & 1     & 1     & 0.9   & 1     & 1     & 1 \\
%\cline{2-8}          & 50-Precision & 0.92  & 0.94  & 0.94  & 0.96  & 0.96  & 0.96 \\
%\cline{2-8}          & 100-Precision & 0.87  & 0.93  & 0.85  & 0.92  & 0.91  & 0.93 \\
%\cline{2-8}          & 200-Precision & 0.84  & 0.9   & 0.845 & 0.875 & 0.855 & 0.86 \\
%    \hline
%    \multirow{4}[8]{*}{Ebola} & 10-Precision & 1     & 1     & 0.8   & 1     & 1     & 1 \\
%\cline{2-8}          & 50-Precision & 0.84  & 0.86  & 0.66  & 0.78  & 0.88  & 0.92 \\
%\cline{2-8}          & 100-Precision & 0.77  & 0.84  & 0.66  & 0.73  & 0.87  & 0.88 \\
%\cline{2-8}          & 200-Precision & 0.765 & 0.8   & 0.61  & 0.71  & 0.86  & 0.87 \\
%    \hline
%    \end{tabular}%
%  \label{tab:eval}%
%\end{table}%




%
%In our scenario we argue that variance and standard deviation are not good measures to represent uncertainty as they have strong positive correlation with the ranking score. Instead, we propose to use VMR to measure uncertainty.
%For a ranking problem, a commonly used correlation coefficient is Spearman's rank correlation coefficient ~\cite{Spearman1904} (short for Spearman's $\rho$). We calculate Spearman's $\rho$ for these three measures between  and run t-test.To show there is little For these three measures, we calculate this coefficient between the ranking score and the uncertainty. Results are shown in Table \ref{Tab:Spearman}.
%
%We can find that Spearman's $\rho$ for variance and standard deviation are all over 0.8, which implies strong positive correlation.
%While the Spearman's $\rho$ of VMR is below 0.2 which shows no significant correlation between ranking scores and uncertainty.
%
%
%\subsection{Retrieval Result Evaluation}
%
%% Table generated by Excel2LaTeX from sheet 'Tables'
%\begin{table}[htbp]
%  \centering
%    \begin{tabular}{|c|r|r|r|r|r|r|r|}
%    \hline
%    \multicolumn{2}{|c|}{\multirow{2}[4]{*}{}} & \multicolumn{2}{c|}{Post} & \multicolumn{2}{c|}{User} & \multicolumn{2}{c|}{Hashtag} \\
%\cline{3-8}    \multicolumn{2}{|c|}{} & Duan's & Ours  & Duan's & Ours  & Duan's & Ours \\
%    \hline
%    \multirow{4}[8]{*}{shutdown} & 10 & 1     & 1     & 0.9   & 1     & 1     & 1 \\
%\cline{2-8}          & 50 & 0.92  & 0.94  & 0.94  & 0.96  & 0.96  & 0.96 \\
%\cline{2-8}          & 100-P & 0.87  & 0.93  & 0.85  & 0.92  & 0.91  & 0.93 \\
%\cline{2-8}          & 200-P & 0.84  & 0.9   & 0.845 & 0.875 & 0.855 & 0.86 \\
%    \hline
%    \multirow{4}[8]{*}{Ebola} & 10-Precision & 1     & 1     & 0.8   & 1     & 1     & 1 \\
%\cline{2-8}          & 50-Precision & 0.84  & 0.86  & 0.66  & 0.78  & 0.88  & 0.92 \\
%\cline{2-8}          & 100-Precision & 0.77  & 0.84  & 0.66  & 0.73  & 0.87  & 0.88 \\
%\cline{2-8}          & 200-Precision & 0.765 & 0.8   & 0.61  & 0.71  & 0.86  & 0.87 \\
%    \hline
%    \end{tabular}%
%  \label{tab:Comparison}%
%  \caption{Add caption}
%\end{table}%
%
%To evaluate the performance of our retrieval model, we compared it with the baseline algorithm proposed by Duan ~\cite{Duan2012_coling}.
%
%We implement our algorithm and the baseline algorithm of ~\cite{Duan2012_coling} by C\#.
%All experiments are done on a PC with a what CPU@3.1GHz and 16 GB RAM.
%
%We use two datasets for the experiments. \textit{Shutdown} and \textit{Ebola}.
%\textit{Shutdown} dataset contains 658385 tweets containing word shutdown during the government shutdown period from October 1, 2013 to October 16, 2013.
%\textit{Ebola} dataset contains 1425017 tweets containing word ebola from January 1, 2014 to December 25, 2014.
%
%As there are too many posts we cannot label all the important posts, users or hashtags. Thus we cannot compare the recall.
%Thus we use n-precision ~\cite{Sieg2007_CIKM} for evaluation. N-precision is the precision of the top n ranked items.
%To fully compare the two algorithms we compare 10,100,1000-precision of posts, users and hashtags.
%The results are shown in Table \ref{}
%
%
%Duan's algorithm may overestimate the importance of some frequent hashtags like:
%its score to more frequent words and users.
%
%\subsection{Incremental Ranking Update Evaluation}
%
%Also we conduct quantitative experiments to show the effectiveness of our incremental ranking update algorithm. We use the retrieval result of our method as a starting point. At each step we modify the ranking score of an item. We document the changes of n-precision. The changes are shown in Figure ???.
%
%We can see that the


==> interaction.tex <==
\section{Interaction}

To better aid users in understanding the inner working mechanism of a CNN and performing deep analysis, CNNvis provides a set of user interactions.

\noindent\textbf{\normalsize Interactive Clustering Result Modification.}
Since the clustering algorithm is less than perfect and users may have different needs, we allow experts to interactively modify the clustering result based on their knowledge (\textbf{R2}).
Inspired by NodeTrix~\cite{Henry2007_Graph}, we allow experts to drag a neuron out of a neuron cluster or to other neuron cluster.

\noindent\textbf{\normalsize Showing Debug Information on Demand.}
Debug information can help experts diagnose a failed training process.
In CNNVis, we allow experts to analyze debug information at different granularity (\textbf{R5}).
% to shixia, not sure whether it is different granularity, but i think so.
For example, as an overview, experts can select to view the average gradient at each layer as a line chart.
They can also change the color encoding of edges to analyze the gradient of each weight.

\noindent\textbf{\normalsize Switching between Multiple Facets of Neurons.}
Exploring multiple facets of neurons can help experts better understand the roles of neurons.
Thus, we allow users to switch between these facets (\textbf{R3}).
For example, users can switch to view the learned features or the activation matrix.
%In addition, users can change the size encoding of neurons to view their contributions or average activations.
%change the size encoding for two of them

\noindent\textbf{\normalsize Selecting A Part of Neorons to View.}
There are thousands of neurons in a CNN.
Thus, it is necessary to allow users to selecting a part of of neurons to view.
In CNNVis, we support several ways to achieve this.
For example, We allow users to select a set of classes and show the neurons which can be strongly activated by the images of these classes.
%from the surface of strongly activated neurons 34 and 35 strongly is more than highly
Other neurons are dehighlighted by setting them translucent.
%The Highlight and Dehighlight combinators
Besides, users can increase or decrease the number of neurons to show in a neurons cluster.





==> overview.tex <==
\begin{figure*}[ht]
  \centering

  \includegraphics[width=\linewidth]{fig/overview}
  \caption{System pipeline: (a) generate evolving topic trees (dotted lines represent matched topics between times); (b) generate evolving tree cuts (the star is the user-selected focus node); (c) reorganize the topics according to the Degree-of-Interest (DOI) values; (d) align topic nodes by their depths; (e) color and scale topic nodes by the DOI values; (f) extract matched documents for the matched topics; (g) generate the final visualization.}\looseness=-1
  \label{fig:overview}
  \vspace{-3mm}
\end{figure*}

\section{Problem Formulation}
Fig.~\ref{fig:overview} briefly illustrates our system pipeline.
The input is a set of documents with time stamps.
First, we extract a sequence of topic trees from the input documents by our evolutionary tree clustering technique, which aims to better organize the topics at different times, as well as match correlated topics between adjacent topic trees.
Second, we transform tree clustering results into a set of salient topics that can well represent the large clustering results and be effectively visualized.
A user selects one or more topics of interest as the focus node(s).
Based on the focus node(s), the tree cut algorithm extracts a set of representative topics for each tree.
The algorithm also makes the representative topic sets at different times coherent with each other.
However, the cut algorithm may still extract too many topics that cannot be clearly displayed on the limited display area.
To tackle this, a mean-shift clustering algorithm~\cite{comaniciu2002mean} is employed to further group the extracted topics.
Meanwhile, the matched documents within the matched topics are extracted based on the relationships between the topics selected by our tree cut algorithm.
Finally, the transformed results, including the topics nodes on each tree cut, matched topics and documents, are visualized for further exploration and analysis.

==> uncertainty.tex <==
%\section{Mutual-Reinforcement-Model-Based Uncertainty Analysis}
%
%\subsection{MRC Computation with a Monte Carlo Method}
%
%\begin{figure}[t]
%  \centering
%  \includegraphics[width=2.5in]{fig/mutual_reinforcement_model}
%  \caption{
%%  \small
%  Mutual reinforcement model.}
%  \label{fig:m_model}
%  \vspace{-3mm}
%\end{figure}
%
%
%
%\subsection{Uncertainty Modeling}
%
%\subsection{Topological Uncertainty Propagation}
%
%%\subsection{Incremental Monte Carlo Method}
%
%\subsection{Incremental Ranking Update}
\section{MRG-Based Uncertainty Analysis}
%In this section, we introduce our solution to MRG.
%\kgsedit{The process of estimating} MRG \kgsedit{exactly is} time-consuming \kgsedit{given} a large graph\kgsedit{; therefore}, we \kgsedit{approximate this graph efficiently using} the Monte Carlo sampling method.
%Since exact inference of MRG is very time-consuming on a large graph, we \kgsedit{approximate this graph efficiently using} the Monte Carlo sampling method.
Since exact inference of MRG is very time-consuming on a large graph, we approximate \shimei{it} using \shimei{a more efficient} Monte Carlo sampling \shimei{method.}
%Accordingly, uncertainty \kgsedit{is} introduced \kgsedit{into MRG}.
%remove by Shimei
%Accordingly, uncertainty will be introduced.
%We explicitly model the uncertainty associated with each item (e.g., a post, a user or a hashtag)\kgsedit{, as} well as its propagation on the graph.
%\shimei{We also} explicitly model the uncertainty associated with each item (e.g., a post, a user or a hashtag)\kgsedit{, as} well as its propagation on the graph.
\shimei{We also} explicitly model the uncertainty associated with each item (e.g., a post, a user\doc{,} or a hashtag)\kgsedit{, as} well as its propagation on the graph.
%We explicitly model the uncertainty associated with each item (e.g., a post, a user or a hashtag) as well as it propagation on the graph.

%\shimeiremove{We provide uncertainty analysis related to the solving process as well} \shimeiremove{as the topological uncertainty propagation. not very sure about} \shimeiremove{what you try to say here.}
%\shimei{not very sure about what you try to say here}
%\mengchen{Mengchen: Here I want to say: As we calculate the ranking scores approximately, . So and enable the users to check high uncertain items. To show the uncertainty we must have an uncertainty model. Besides, we calculate the ranking scores on a graph. Thus the uncertainty will propagate on the graph. Thus if an item is high uncertain, its neighbours will probably be uncertain. We want to model this uncertainty propagation on graph.}


\subsection{MRG Computation with Monte Carlo Sampling Method}

%Duan et al.~\cite{Duan2012_coling} proposed a matrix-based method to solve \kgsedit{MRG. This method} iteratively updates the ranking scores using Eq.~(\ref{eq:4.1}). The matrix-based method is a global \kgsedit{;}
Duan et al.~\cite{Duan2012_coling} proposed a matrix-based method to solve MRG, which iteratively updates the ranking scores using Eq.~(\ref{eq:4.1}).
%The matrix-based method is a global method.
The matrix-based method is a global \doc{one}.
%\kgsedit{however, items are updated} by running the \kgsedit{process} on the \kgsedit{entire} item \kgsedit{set. This procedure is time-consuming.}
%An update to any item is achieved by running the method on the whole item set, which is very time-consuming.
An update to any item is achieved by running the method on the \shimei{entire} item set, which is very \shimei{time-consuming.}
%As a result, an efficient method with local \kgsedit{updating capability is needed in} our system to \kgsedit{support} interactive modification.
%remove by Shimei
%As a result, an efficient method with local update is needed in our system to support the interactive modification.
To \kgsedit{address} this problem, we use the Monte Carlo sampling \kgsedit{method}.
%To solve this problem, we use Monte Carlo sampling methods.
\kgsedit{The} advantages of \kgsedit{this} sampling method \kgsedit{over the matrix-based method are as follows}~\cite{Avrachenkov2007}:
%Comparing to matrix-based method, the advantages of the Monte Carlo sampling method includes~\cite{Avrachenkov2007}:
\begin{compactitem}
\item \kgsedit{Ranking} scores \kgsedit{are locally updated} when the input changes locally;
%\item Allow local update of ranking scores when the input changes locally;
\item \kgsedit{The} ranking scores of important items \kgsedit{are accurately estimated} after a few iterations;
%\item Accurately estimate the ranking scores of important items after a few iterations;
\item \kgsedit{The} uncertainty of the ranking scores \kgsedit{are modeled} accurately because \kgsedit{the Monte Carlo} method calculates variance statistically.
%\item Model the uncertainty of the ranking scores more accurately because this method calculates variance statistically.
\end{compactitem}

To employ \kgsedit{this} \kgsedit{method}, we first solve $R$ \kgsedit{as formulated} by Eq.~(\ref{eq:4.2}):
%To employ Monte Carlo sampling methods, we first solve $R$ from Eq.~(\ref{eq:4.2}):

%In our work we adopt a Monte Carlo sampling method to solve the MRG.

%\shimei{Shimei: is the method used here the same as that in [3]? If so, we need to reword it so that it is clear.}
%\mengchen{Mengchen: Yes, it is the same.}
%The Monte Carlo sampling methods are probabilistic methods that take repeated random samples and use statistics of the samples to estimate numerical results.

\begin{equation}
\small
\label{eq:5.1.1}
R  = (1 - d)(I - dM)^{ - 1}W  = (1 - d)(\sum\limits_{k = 0}^\infty  {d^k M^k })W.
\end{equation}

%\kgsedit{We then} perform a series of random walks $\{ X_t \} ,t \ge 0$ \kgsedit{for each item}.
\revision{We then perform a series of random walks for each item.}
%Then for each item, we perform a series of random walks $\{ X_t \} ,t \ge 0$.
A random walk may stop at each step with a probability of $1 - d$.
If \kgsedit{the walk} continues, \kgsedit{then it proceeds} to the next step according to the matrix $M$.
%If it continues, it will move to the next step according to the matrix $M$.
Each element $m_{ij} $ defines the transition probability from $i$ to $j$.

Let \begin{small}$Z = \sum\limits_{k = 0}^\infty  {d^k M^k }$\end{small}\kgsedit{. The} ranking score of each item is:
%Let $Z = \sum\limits_{k = 0}^\infty  {d^k M^k }$, the ranking score of each item is:
\begin{equation}
\small
\label{eq:5.1.2}
r_j  = (1 - d)\sum\limits_{i = 1}^N {w_i z_{ij} },
\end{equation}
%where the element $z_{ij} $ in $Z$ is the average number of times that the random walk \kgsedit{starting from item $i$} visits item $j$.
where the element $z_{ij} $ in $Z$ is the average number of times that \shimei{a} random walk starting from item $i$ visits item $j$.
%\revision{where $z_{ij} $ in $Z$ is the average number of times of the random walks that starts from item $i$ and visits item $j$.}
We estimate $z_{ij}$ by computing the empirical mean of a number of random walks.
%To estimate $Z_{ij}$ we first take a lot of random walks and then use the empirical mean as an estimate of $Z_{ij}$.
%To speed up the algorithm, we adopt the sampling strategy in~\cite{Avrachenkov2007} where we use the whole path to estimate $Z_{ij}$.

%\mengchen{Mengchen: not sure if we should add the improvement of using path more efficiently}
Duan et al.~\cite{Duan2012_coling} \kgsedit{only consider} the similarity of items \kgsedit{in computing} $m_{ij}$.
%Duan et al.~\cite{Duan2012_coling} only use the similarity of items to compute $m_{ij}$.
%\kgsedit{Thus, high-ranking} scores \kgsedit{may be incorrectly assigned to} users who publishes \kgsedit{many} posts \kgsedit{that do not receive} attention.
\kgsedit{Thus, high-ranking} scores \kgsedit{may be incorrectly assigned to} users who \doc{publish} \kgsedit{many} posts \kgsedit{that do not receive} attention.
%This may wrongly assign high ranking scores to these users who publishes a lot of posts with no attention.
To \kgsedit{address} this, we \kgsedit{consider the} prior saliency of \kgsedit{items} in the sampling \kgsedit{process}.
%To solve this problem, we take prior saliency of items into consideration in the sampling.
Specifically, the transition probability from $m_{ij}$ is defined as $similarity(i,j) \cdot w_j$.
%By incorporating prior saliency we can

\subsection{Uncertainty Modeling}

%\kgsedit{We} use an approximation to solve \kgsedit{MRG;} \kgsedit{therefore,} the retrieval result \kgsedit{in uncertain}.
%\revision{In MutualRanker, we use an approximation to solve MRG,
%\revision{In MutualRanker, we use an approximation \shimei{method} to solve MRG, which may introduce uncertainty into the retrieval result.
\revision{In MutualRanker, we use an approximation \shimei{method} to solve MRG, which may introduce uncertainty into the retrieval result\doc{s}.
%As a result, \kgsedit{model} uncertainty \kgsedit{must be modeled} accurately.
It is therefore important to model uncertainty.
%\kgsedit{Probability, fuzzy set, rough set, and evidence theories} are the major frameworks \kgsedit{used} to model uncertainty ~\cite{Zimmermann2001fuzzy}. \kgsedit{Specifically, probability} theory is commonly \kgsedit{applied} when the distribution of the measured values \kgsedit{is} known.
%Probability theory, fuzzy set theory, rough set theory, and evidence theory are the major frameworks to model uncertainty ~\cite{Zimmermann2001fuzzy}.
%Specifically, probability theory is commonly used when the distribution of the measured values is known.
%Probability theory is commonly used when the distribution of the measured values is known.
%\kgsedit{We utilize the} Monte Carlo sampling \kgsedit{method; thus,} the distribution of each ranking score is known.
Since we employ the Monte Carlo sampling method, the distribution of each ranking score is \shimei{known.}
%Probability theory is commonly used when the distribution of the measured value is known.
%remove by shimei
%Hence, we employ probability theory to model uncertainty.}\looseness=-1
\shimei{Hence,} we \shimei{can} employ \shimei{the} probability theory to model uncertainty.}\looseness=-1
%Thus, we employ the probability theory to model the uncertainty.

%According to~\cite{BIPM1995}, uncertainty is defined as a parameter \kgsedit{to depict the} dispersion of \kgsedit{values} that can \kgsedit{be reasonably} attributed to the measured value.
%According to~\cite{BIPM1995}, 
\doc{Uncertainty is defined as a parameter for depicting} the dispersion of \kgsedit{values} that can \kgsedit{be reasonably} attributed to the measured value~\cite{BIPM1995}.
%According to~\cite{BIPM1995}, uncertainty is defined as a parameter to depicts the dispersion of the values that can reasonably be attributed to the measured value.
Traditional methods model the measured value as a normally distributed random variable~\cite{Correa2009_VAST,Wu2012_InfoVis}.
Variance~\cite{Correa2009_VAST} and standard deviation~\cite{Wu2012_InfoVis} are \kgsedit{among the most} commonly used measures to represent \kgsedit{uncertainty wherein} the measured value is defined on the set of both positive and negative real numbers.
%Variance~\cite{Correa2009_VAST} and standard deviation~\cite{Wu2012_InfoVis} are two commonly used measures to represent uncertainty,in which the measured value is defined on the set of both positive and negative real numbers.

%The measured value (\kgsedit{ranking} score) in our approach is defined on the set of positive real numbers, \kgsedit{thus, }the above modeling method cannot be \kgsedit{applied directly} to our work.
The measured value (\kgsedit{ranking} score) in our approach is defined on the set of positive real numbers\doc{. Thus, }the above modeling method cannot be \kgsedit{applied directly} to our work.
%Since the measured value (the ranking score) in our approach is defined on the set of positive real numbers, the above modeling method cannot be directly applied to our work.
%As a result, we employ the negative binomial dispersion parameter to model uncertainty.

%In Eq.~(\ref{eq:5.1.2}), $z_{ij}$ represents the average times that \kgsedit{a} random walk starting at $i$ visits $j$.
%In Eq.~(\ref{eq:5.1.2}), $z_{ij}$ represents the average \doc{number of} times that \kgsedit{a} random walk starting at $i$ visits $j$.
\revision{According to~\cite{Avrachenkov2007}, $z_{ij}$ in Eq.~(\ref{eq:5.1.2}) has a Poisson distribution.}
%In Eq.~(\ref{eq:5.1.2}), $z_{ij}$ represents the average times that a random walk starts at $i$ and visits $j$. According to~\cite{Avrachenkov2007} $z_{ij}$ has a Poisson distribution.
The ranking score is the weighted sum of a series of $z_{ij} $.
\kgsedit{Hence}, the ranking score is modeled as a Poisson mixture.
%As a result, the ranking score is modeled as a Poisson mixture.
For \kgsedit{a} Poisson \kgsedit{mixture,} the variance is approximately proportional to the \kgsedit{mean. Hence, if} we use variance to model uncertainty, the larger \kgsedit{the} ranking \kgsedit{score}, the more uncertain it is, \kgsedit{but this is} not always true.
%For Poisson mixture the variance is approximately proportional to the mean.If we use variance to model uncertainty, the larger a ranking score is, the more uncertain it is, which is not always true.

Standard deviation is the square root of variance and has \kgsedit{a} similar problem.
%Standard deviation is the square root of variance and has the similar problem.
%\kgsedit{Consequently,} variance and standard deviation are not good measures to depict uncertainty in our scenario.
%Consequently, variance and standard deviation are not good measures to depict uncertainty in our \shimei{model}.
Consequently, variance and standard deviation are not good measures \doc{for depicting} uncertainty in our \shimei{model}.
%Consequently variance and standard deviation are not good measures to depict uncertainty in our scenario.

%For such distribution, a commonly used measure to depict the dispersion is the variance-mean-ratio (VMR)~\cite{Cox1966}. The higher the \kgsedit{VMR}, the more dispersed \kgsedit{the distribution}. For item $j$, its VMR ($u_j$) can be defined as:\looseness=-1
For such \shimei{a} distribution, a commonly used measure \shimei{of} dispersion is the variance-mean-ratio (VMR)~\cite{Cox1966}. The higher the \kgsedit{VMR}, the more dispersed \kgsedit{the distribution}. For item $j$, its VMR ($u_j$) can be defined as:\looseness=-1
%For such distribution, a commonly used measure to depict the dispersion is the variance-mean-ratio (VMR)~\cite{Cox1966}. The higher VMR is, the more dispersed a distribution is. For item $j$, its VMR ($u_j$) can be defined as follows:

\begin{equation}
\small
\label{eq:5.2.1}
u_j  = {{v_j }}/{{r_j }} ,
\end{equation}
where $v_j $ is the distribution variance of the ranking score of item $j$.
%As $u_j$ can depict the dispersion of this distribution,
%for an item $j$, we can use $u_j$ to measure the uncertainty of its ranking score.
According to~\cite{Avrachenkov2007}, $v_j$ can be calculated as follows:

\begin{equation}
\small
v_j  = (1 - d)^2 \sum\limits_{i = 1}^N {w_i^2 v_{z_{ij}}}.
\end{equation}
where $v_{z_{ij}}$ is the variance of ${z_{ij}}$. \kgsedit{Each} $z_{ij}$ obeys a Poisson distribution \kgsedit{and its} variance can be calculated from its expectation.
%where $v_{z_{ij}}$ is the variance of ${z_{ij}}$. As each $z_{ij}$ obeys a Poisson distribution, its variance can be calculated from its expectation.
%Here we approximately use the empirical mean as expectation.
%After calculating the variance of the ranking score of each item,
%Then we can use Eq.~(\ref{eq:5.2.1}) to calculate the uncertainty of the ranking scores.

%\kgsedit{The abundance of items in the} microblog data \kgsedit{means} we cannot place all of them on the screen. \kgsedit{Hence, we} aggregate similar items to form a cluster. The overall ranking score of a cluster, $r_c$\, is defined as the sum of ranking scores of its items~\cite{Bianchini2005}.
The \shimei{massive number} of items in the microblog data \kgsedit{means} we cannot place all of them on the screen.
\kgsedit{Hence, we} aggregate similar items to form a cluster.
%The overall ranking score of a cluster, $r_c$\, is defined as the sum of \shimei{the} ranking scores of its items~\cite{Bianchini2005}.
The overall ranking score of a \doc{cluster $r_c$} is defined as the sum of \shimei{the} ranking scores of its items~\cite{Bianchini2005}.
%Since there are too many items in microblog data, we cannot place all of them on the screen. We then aggregate similar items to form a cluster. The overall ranking score of a cluster $r_c$ is defined as the sum of ranking scores of its items~\cite{Bianchini2005}.
%The ranking scores are independent \kgsedit{of} each other, \kgsedit{and the} overall variance of the cluster, $v_c$, is the sum of the variance of the ranking scores. \kgsedit{Thus,} the uncertainty of a cluster, $u_c$, can be \kgsedit{calculated naturally} by dividing $v_c$ and $r_c$.
The ranking scores are independent \kgsedit{of} each \doc{other and} the overall variance of the cluster, $v_c$, is the sum of the variance of the ranking scores. \kgsedit{Thus,} the uncertainty of a cluster, $u_c$, can be \kgsedit{calculated naturally} by dividing $v_c$ and $r_c$.
%The ranking scores are independent with each other, the overall variance of the cluster $v_c$ is the sum of the variance of the ranking scores. Thus the uncertainty of a cluster $u_c$ can be naturally calculated by dividing $v_c$ and $r_c$.

\begin{equation}
\small
\label{eq:5.2.2}
{{u}_{c}}={{{v}_{c}}}/{{{r}_{c}}}=\sum\limits_{j\in c}{(r_j/r_c)(v_j/r_j)}=\sum\limits_{j\in c}{{{k}_{j}}{{u}_{j}}}.
\end{equation}
%\kgsedit{Eq.~(\ref{eq:5.2.2}) shows that} $u_c$ can be expressed by \kgsedit{the} weighted sum of the uncertainty of its items where each weight $k_j$ is the ratio of the ranking scores of item $j$ and \kgsedit{cluster} $c$.
\kgsedit{Eq.~(\ref{eq:5.2.2}) shows that} $u_c$ can be expressed by \doc{a} weighted sum of the uncertainty of its items where each weight $k_j$ is the ratio of the ranking scores of item $j$ and \kgsedit{cluster} $c$.
%From Eq.~(\ref{eq:5.2.2}) we can see that $u_c$ can be expressed by a weighted sum of the uncertainty of its items where each weight $k_j$ is the ratio of the ranking scores of item $j$ and the cluster $c$.
\kgsedit{Thus,} the uncertainty of a cluster is \kgsedit{mainly determined} by its important items.

\subsection{Topological Uncertainty Propagation}
\label{sec:propagation}

%\revision{If an analyst finds an incorrect ranking, he can modify it based on his knowledge.
\revision{If an analyst finds an \shimei{incorrectly ranked item}, he can modify it based on his knowledge.
%He can further track how the uncertainty propagates from one cluster to another for identifying more uncertain items.}
He can further track how the uncertainty propagates from one cluster to another \shimei{to identify other affected} items.}
%\kgsedit{We} explicitly model its topological propagation on the graph \kgsedit{to assist in tracking the uncertainty}.
%To help the analyst track uncertainty, we explicitly model its topological propagation on the graph.
To help \shimei{an} analyst track uncertainty, we explicitly model its topological propagation on the graph.

In MRG, the ranking score of an item can be expressed as a linear combination \kgsedit{of} ranking scores of related items.
%In MRG, the ranking score of an item can be expressed as a linear combination of the ranking scores of related items.
\kgsedit{Hence}, the variances of a ranking score can also be expressed as a linear combination of the variances \kgsedit{of} related ranking scores.
%As a result, the variances of a ranking score can also be expressed as a linear combination of the variances of the related ranking scores.
\kgsedit{The} uncertainty of each item can be calculated from its ranking score and its variance, \kgsedit{and hence,} the uncertainty of an item can also be \kgsedit{expressed linearly by the} uncertainty of other items. \kgsedit{Specifically,}
%As the uncertainty of each item can be calculated from its ranking score and its variance, the uncertainty of an item can also be linearly expressed by uncertainty of other items. Specifically

\begin{equation}
\small
\label{eq:5.3.1}
u_j  = \sum\limits_{i = 1,i \ne j}^N {m_{ij}^* u_i },
\end{equation}
%where each $m_{ij}^* = ({d^2 m_{ij}^2 r_i })/({(1 - d^2 m_{jj} )r_j })$. \kgsedit{Eq.~(\ref{eq:5.3.1}) shows that the} uncertainty of each item is not independent and \kgsedit{propagates} on the graph in a linear form.
where each $m_{ij}^* = ({d^2 m_{ij}^2 r_i })/({(1 - d^2 m_{jj} )r_j })$. \kgsedit{Eq.~(\ref{eq:5.3.1}) shows that the} uncertainty of each item is not independent and \shimei{it} \kgsedit{propagates} on the graph in a linear form.
%where each $m_{ij}^* = \frac{{d^2 m_{ij}^2 r_i }}{{(1 - d^2 m_{jj} )r_j }}$. From Eq.~(\ref{eq:5.3.1}) we can see that uncertainty of each item is not independent and propagate on the graph in a linear form.
\kgsedit{Thus,} for each pair of items $i$ and $j$, $m_{ij}^* u_i $ can be viewed as the propagated uncertainty from item $i$ \kgsedit{to} $j$. We denote it by $u_{i \to j}$.
%Thus for each pair of items $i$ and $j$, $m_{ij}^* u_i $ can be viewed as the propagated uncertainty from item $i$ to item $j$. We denote it by $u_{i \to j}$.

Rewriting Eq.~(\ref{eq:5.3.1}) in a matrix form, we can formulate the uncertainty propagation as a Markov chain:

\begin{equation}
\small
UM^*  = U,
\end{equation}
where $U = [u_j]_{1 \times N}$ and $M^* = [m_{ij}^*]_{N \times N}$.

Similar to the uncertainty propagation from item to item, we can model the uncertainty propagation from cluster to cluster using the following procedure.
%First, \kgsedit{we} calculate the propagated uncertainty from each item $i$ \kgsedit{in} source cluster $c_s$ to each item $j$ in the target cluster $c_t$ \kgsedit{based on Eq.~(\ref{eq:5.3.1})}(Fig.~\ref{fig:uncertainty_2}(a)).
First, based on Eq.~(\ref{eq:5.3.1}), we calculate the propagated uncertainty from each item $i$ in the source cluster $c_s$ to each item $j$ in the target cluster $c_t$ (Fig.~\ref{fig:uncertainty_2}(a)).
Second, for each item $j$ in $c_t$, we compute the propagated uncertainty $u_{c_s \to j}$ from $c_s$ to item $j$ by aggregating the uncertainty propagated from each item in the source cluster (Fig.~\ref{fig:uncertainty_2}(b)).

\begin{equation}
\small
u_{c_s \to j}  = \sum\limits_{i \in c_s } {u_{i \to j} }.
\end{equation}
Finally, the uncertainty of a cluster is a weighted sum of the uncertainty of the items in it (Eq.~(\ref{eq:5.2.2})).
\kgsedit{Thus,} the overall propagated uncertainty $u_{c_s \to c_t}$ from $c_s$ to $c_t$ can be calculated as \kgsedit{the} weighted sum of the propagated uncertainty from $c_s$ to each $j$ in $c_t$ (Fig.~\ref{fig:uncertainty_2}(c)).
%Thus the overall propagated uncertainty $u_{c_s \to c_t}$ from $c_s$ to $c_t$ can be calculated as a weighted sum of the propagated uncertainty from $c_s$ to each $j$ in $c_t$.

%The weight is proportional to the ranking score of the target item.

%Finally, the uncertainty of the target community can be expressed as a weighted sum of the uncertainty of the items in it (shown in Figure~\ref{fig:uncertainty_2}(c))

\begin{equation}
\small
u_{c_s \to c_t}  = \sum\limits_{j \in c_t } {k_j u_{c_s \to j} }.
\end{equation}

\begin{figure}[t]
  \centering
  \includegraphics[width=0.45\textwidth]{fig/uncertainty-2}
  \vspace{-3mm}
  \caption{
%  \small
  Topological uncertainty propagation calculation}
  \label{fig:uncertainty_2}
  \vspace{-5mm}
\end{figure}

%\subsection{Incremental Monte Carlo Method}

\subsection{Incremental Ranking Update}

%We also allow analysts to modify the item ranking \kgsedit{results interactively} based on their knowledge.
We also allow analysts to interactively modify the item ranking result based on their knowledge.
\kgsedit{We can update the model locally because we} use the Monte Carlo sampling method.
%Since we use Monte Carlo sampling methods, we can update the model locally.
%\kgsedit{After} the analyst changes the ranking score(s), our approach iteratively updates the prior salience of the item(s).
\kgsedit{After} the analyst changes the ranking score(s), our approach iteratively updates the prior salience \shimei{score(s)} of the item(s).
%Specifically, after the analyst changes the ranking score(s), our approach iteratively update the prior salience of the item(s).
Accordingly, the affinity matrix is changed from $M$ to $M'$.
%This change affects a small part of \kgsedit{the} random walks \kgsedit{used in the} Monte Carlo sampling method.
This change \shimei{only} affects a small part of \kgsedit{the} random walks \kgsedit{used in the} Monte Carlo sampling method.
%This change affects a small part of random walks that we used in the Monte Carlo sampling methods.

For \kgsedit{the} affected random walks, existing incremental graph ranking algorithms ~\cite{Bahmani2010} perform re-sampling and update the ranking scores by aggregating the statistics of these new random walks into the original \kgsedit{results}.
%For those affected random walks, existing incremental graph ranking algorithms ~\cite{Bahmani2010} perform re-sampling and update the ranking scores by aggregating the statistics of these new random walks into the original result.
%The main problem of these algorithms is that re-sampling \kgsedit{involves considerable} time and \kgsedit{the requirements of real-time interaction may not be met}.
%\shimei{One} main problem of these algorithms is that re-sampling \shimei{requires} considerable \shimei{amount of} time \shimei{which may make} real-time interaction \shimei{impossible}.
\shimei{One} main problem \doc{with} these algorithms is that re-sampling \shimei{requires} \doc{a} considerable \shimei{amount of} time\doc{,} \shimei{which may make} real-time interaction \shimei{impossible}.
%The main problem of these algorithms is that re-sampling takes a lot of time and may not meet the requirement of real-time interaction.
%Suppose $n$ is the average number of neighbors of an item and $l$ is the average length of a sampled random walk.
Suppose $n$ is the average number of neighbors that an item \shimei{has} and $l$ is the average length of a sampled random walk.
At each step in a random walk, we have to sample from a multinomial distribution with $n$ possible outcomes and the time cost is $O(n)$.
%Thus sampling a new random walk will take $O(nl)$ time.
Thus\doc{,} sampling a new random walk will take $O(nl)$ time.
\kgsedit{The} time needed \kgsedit{to compute and aggregate the} statistics of \kgsedit{these} samples is $O(l)$.
%Thus, the total time cost for a new sample is $O(nl) + O(l)=O(nl)$.
%Thus, the total time \shimei{required} for a new sample is $O(nl) + O(l)=O(nl)$.
\doc{The} total time \shimei{required} for a new sample is $O(nl) + O(l)=O(nl)$.
%In addition, the time needed in computing and aggregating statistics of this samples is $O(l)$. Thus the total time cost for a new sample is $O(nl) + O(l)=O(nl)$.

However, in our scenario, we do not \kgsedit{delete} or add edges on the graphs.
%However, in our scenario, we do not delete edges or add edges on the graphs.
%As a result, we \kgsedit{(need to be checked)do not} need to perform \kgsedit{re-sampling}.
As a result, we do not need to perform re-sampling.
%Using this feature, we only modify the statistics of a random walk based on the modified transition probability $m_{ij}$\kgsedit{, thereby} avoiding the high cost sampling procedure.
\shimei{We} only \shimei{need to} modify the statistics of a random walk based on the modified transition probability $m_{ij}$, thereby avoiding the high cost \shimei{associated with resampling.}
%Using this feature, we only modify the statistics of a random walk based on the modified transition probability $m_{ij}$ and thus avoiding the high cost sampling procedure.
The time cost of updating an influenced random walk is reduced to $O(l)$.

%Here we don't re-sample the items in our graph. Instead, for each affected sample we only change its  we only modify the transition weights associated with an influenced sample.

%Thus we can save the time of re-sampling. Suppose $l$ is the average length of a random walk
%which is $\frac{1}{1-d}$
%and $n$ is the average number of neighbors of an item.  Thus the time needed for resampling is $O(nl)$. In contrast, the time needed in computing statistics of existing samples is $O(l)$.
%\shimei{Commnet from Shimei: I am not sure about the meaning of this statement}.
%\mengchen{Mengchen: For Monte Carlo methods, there are two steps. The first is take samples. The second is to aggregate the samples such as calculate the mean of the samples. For the old update methods, they need to take new samples for the influenced samples and aggregate the new samples. In our algorithm we only need to change the weight of influenced samples. Thus we can save the time of resampling. While taking a new sample may cost much longer time than aggregating a sample. So we can save a lot of time.}
%Thus the time complexity of our algorithm is only O(1/n) of those that require new samples

Given a random walk: $path = \{ i \to n_1  \to ... \to n_{k - 1}  \to j\}$, we define a new random variable $x_{ij}^{k} $.
In particular, $x_{ij}^{k}  = 1$ indicates \kgsedit{that} the random walk \kgsedit{starts} from $i$ and \kgsedit{reaches} $j$ by moving $k$ steps.
%Given a random walk: $path = \{ i \to n_1  \to ... \to n_{k - 1}  \to j\}$, we define a new random variable $x_{ij}^{k} $. $x_{ij}^{k}  = 1$, which indicates the random walk starting from $i$ and reaching $j$ by moving $k$ steps.
The original weight of each step in the random walk is $1$.
%During \kgsedit{an} update, we re-calculate the weight of this step \kgsedit{through} ${{P'(x_{ij}^{k}  = 1)}}/{{P(x_{ij}^{k}  = 1)}}$.
During \kgsedit{an} update, we re-calculate the weight of this step \shimei{using} ${{P'(x_{ij}^{k}  = 1)}}/{{P(x_{ij}^{k}  = 1)}}$.
%The original weight of each step in the random walk is $1$.  During update, we re-calculate the weight of this step using $\frac{{P'(x_{ij}^{k}  = 1)}}{{P(x_{ij}^{k}  = 1)}}$.
$P(x_{ij}^{k}  = 1)$ is the probability of $x_{ij}^{k}  = 1$ according to $M$ and $P'(x_{ij}^{k}  = 1)$ is the probability of $x_{ij}^{k}  = 1$ according to $M'$.
\kgsedit{Hence,} $P(x_{ij}^{k}  = 1)$ is calculated by:
%$P(x_{ij}^{k}  = 1)$ can be calculated by.

\begin{equation}
\small
\label{eq:5.4.1}
P(x_{ij}^{k}  = 1) = m_{in_1 } m_{n_1 n_2 } ...m_{n_{k - 1} j}.
\end{equation}
%\kgsedit{$P'(x_{ij}^{k}  = 1)$ }can also be calculated.
Similarly, $P'(x_{ij}^{k}  = 1)$ can also be calculated. 
